Meta-Learning for Few-Shot Time Series Classification

Deep neural networks (DNNs) have achieved state-of-the-art results on time series classification (TSC) tasks. In this work, we focus on leveraging DNNs in the often-encountered practical scenario where access to labeled training data is difficult, and where DNNs would be prone to overfitting. We leverage recent advancements in gradient-based meta-learning, and propose an approach to train a residual neural network with convolutional layers as a meta-learning agent for few-shot TSC. The network is trained on a diverse set of few-shot tasks sampled from various domains (e.g. healthcare, activity recognition, etc.) such that it can solve a target task from another domain using only a small number of training samples from the target task. Most existing meta-learning approaches are limited in practice as they assume a fixed number of target classes across tasks. We overcome this limitation in order to train a common agent across domains with each domain having different number of target classes, we utilize a triplet-loss based learning procedure that does not require any constraints to be enforced on the number of classes for the few-shot TSC tasks. To the best of our knowledge, we are the first to use meta-learning based pre-training for TSC. Our approach sets a new benchmark for few-shot TSC, outperforming several strong baselines on few-shot tasks sampled from 41 datasets in UCR TSC Archive. We observe that pre-training under the meta-learning paradigm allows the network to quickly adapt to new unseen tasks with small number of labeled instances.

==> rl_math.tex <==
% GENL MATH
\newcommand{\Real}{\mathbb{R}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\given}[1][]{\:#1\vert\:}
\newcommand{\givenb}{\:\middle\vert\:}
\newcommand{\suchthat}{\:\vert\:}
\newcommand{\grad}{\nabla}
\newcommand{\evalat}[1]{\big\rvert_{#1}}

% STATISTICS
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Ea}[1]{\E\left[#1\right]}
\newcommand{\Eb}[2]{\E_{#1}\left[#2\right]}
\newcommand{\Vara}[1]{\Var\left[#1\right]}
\newcommand{\Varb}[2]{\Var_{#1}\left[#2\right]}
\newcommand{\lone}[1]{\norm{#1}_1}
\newcommand{\Prob}[1]{\operatorname{Pr}\left[#1\right]}

% NORMS
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\abs}{|}{|}
\newcommand{\pospart}[1]{\abs{#1}^+}
\DeclarePairedDelimiter{\lrbrack}{[}{]}
\DeclarePairedDelimiter{\lrbrace}{ \{ }{ \} }
\DeclarePairedDelimiter{\lrparen}{(}{)}
\DeclarePairedDelimiter{\lrang}{\langle}{\rangle}
\newcommand{\infnorm}[1]{\norm{#1}_{\infty}}
\newcommand{\normone}[1]{\norm{#1}_1}

% MDP
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\adv}{\mathbb{A}}
\newcommand{\rhopi}{\rho_{\pi}}
\newcommand{\Qpi}{\ensuremath{Q^{\pi}}}
\newcommand{\Api}{\ensuremath{A^{\pi}}}
\newcommand{\Vpi}{\ensuremath{V^{\pi}}}
\newcommand{\Qstar}{\ensuremath{Q^{*}}}
\newcommand{\Astar}{\ensuremath{A^{*}}}
\newcommand{\Vstar}{\ensuremath{V^{*}}}

% DIVERGENCE
\newcommand{\kl}[2]{D_{KL}\left[#1 ~ \| ~ #2\right]}
\newcommand{\tv}[2]{D_{TV}(#1 \ \| \ #2)}

% MISC
\newcommand{\tdlam}{TD($\lambda$)}
\newcommand{\tdzero}{TD($0$)}
\newcommand{\tdone}{TD($1$)}
\newcommand{\lstdlam}{LSTD($\lambda$)}
\newcommand{\lstdzero}{LSTD($0$)}
\newcommand{\lstdone}{LSTD($1$)}
\newcommand{\brmlam}{BRM($\lambda$)}
\newcommand{\brmzero}{BRM($0$)}
\newcommand{\brmone}{BRM($1$)}
\newcommand{\lspelam}{LSPE($\lambda$)}
\newcommand{\lspezero}{LSPE($0$)}
\newcommand{\lspeone}{LSPE($1$)}
\newcommand{\qlrn}{$Q$-learning}
\newcommand{\qfcn}{$Q$-function}
\newcommand{\sarsalam}{SARSA($\lambda$)}
\newcommand{\gaelam}{GAE($\lambda$)}
\newcommand{\sarsazero}{SARSA($0$)}
\newcommand{\watq}{Watkins' $Q$-learning}
\newcommand{\myint}[1]{\int \! \! \mathrm{d} #1 \ }

